Work-Efficient Parallel Non-Maximum Suppression Kernels

In the context of object detection, sliding-window classifiers and single-shot Convolutional Neural Network (CNN) meta-architectures typically yield multiple overlapping candidate windows with similar high scores around the true location of a particular object. Non-Maximum Suppression (NMS) is the process of selecting a single representative candidate within this cluster of detections, so as to obtain a unique detection per object appearing on a given picture. In this paper, we present a highly scalable NMS algorithm for embedded GPU architectures that is designed from scratch to handle workloads featuring thousands of simultaneous detections on a given picture. Our kernels are directly applicable to other sequential NMS algorithms such as FeatureNMS, Soft-NMS or AdaptiveNMS that share the inner workings of the classic greedy NMS method. The obtained performance results show that our parallel NMS algorithm is capable of clustering 1024 simultaneous detected objects per frame in roughly 1 ms on both NVIDIA Tegra X1 and NVIDIA Tegra X2 on-die GPUs, while taking 2 ms on NVIDIA Tegra K1. Furthermore, our proposed parallel greedy NMS algorithm yields a 14x-40x speed up when compared to state-of-the-art NMS methods that require learning a CNN from annotated data.

==> references.tex <==
%------------------------------------
% Bibliography
%------------------------------------

@inproceedings{oro2016work,
  title={{{Work-efficient Parallel Non-maximum Suppression for Embedded GPU Architectures}}},
  author={Oro, David and Fern{\'a}ndez, Carles and Martorell, Xavier and Hernando, Javier},
  booktitle={IEEE International Conference on Acoustics, Speech and Signal Processing},
  address={Shanghai, China},
  pages={1026--1030},
  year={2016},
  organization={IEEE, Piscataway, NJ, USA}
}

@inproceedings{liu2016ssd,
  title={{{SSD: Single Shot Multibox Detector}}},
  author={Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C},
  booktitle={European Conference on Computer Vision},
  address={Amsterdam, The Netherlands},
  publisher={Springer, Berlin},
  pages={21--37},
  year={2016}
}

@inproceedings{lin2014microsoft,
  title={{{Microsoft COCO: Common Objects in Context}}},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle={European Conference on Computer Vision},
  address={Zurich, Switzerland},
  pages={740--755},
  publisher={Springer, Berlin},
  year={2014}
}

@manual{armbiglittle,
  title={{{Arm big.LITTLE}}},
  author={{Arm Ltd.}},
  note={\url{https://developer.arm.com/technologies/big-little}},
  year={2019}
}

@article{zhang2016joint,
  title={{{Joint Face Detection and Alignment Using Multitask Cascaded Convolutional Networks}}},
  author={Zhang, Kaipeng and Zhang, Zhanpeng and Li, Zhifeng and Qiao, Yu},
  journal={IEEE Signal Processing Letters},
  volume={23},
  number={10},
  pages={1499--1503},
  year={2016},
  publisher={IEEE}
}

@inproceedings{li2015convolutional,
  title={{{A Convolutional Neural Network Cascade for Face Detection}}},
  author={Li, Haoxiang and Lin, Zhe and Shen, Xiaohui and Brandt, Jonathan and Hua, Gang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  address={Boston, MA, USA},
  pages={5325--5334},
  publisher={IEEE Computer Society, Washington D.C., USA},
  year={2015}
}

@manual{nvidiaxaviersite,
  title={{{NVIDIA Jetson Xavier}}},
  author={{NVIDIA Corp.}},
  note={\url{https://developer.nvidia.com/jetson-xavier}},
  year={2019}
}

@manual{nvidiaarchs,
  title={{{NVIDIA Architectures}}},
  author={{NVIDIA Corp.}},
  note={\url{https://www.nvidia.com/page/products.html}},
  year={2020}
}

@inproceedings{volta18ipdps,
  title={{{NVIDIA Tensor Core Programmability, Performance and Precision}}},
  author={Markidis, Stefano and Chien, Der and Wei, Steven and Laure, Erwin and Bo Peng, Ivy and Vetter, Jeffrey S.},
  booktitle={Proceedings of the IEEE International Parallel and Distributed Processing Symposium Workshops},
  address={Vancouver, BC, Canada},
  publisher={IEEE, Piscataway, NJ, USA},
  year={2018}
}

@inproceedings{angelovareal,
  title={{{Real-Time Pedestrian Detection With Deep Network Cascades}}},
  author={Angelova, Anelia and Krizhevsky, Alex and Vanhoucke, Vincent and Ogale, Abhijit and Ferguson, Dave},
  booktitle={Proceedings of the British Machine Vision Conference},
  address={Swansea, UK},
  publisher={BMVA Press, Durham, UK},
  year={2015}
}

@inproceedings{girshick2014rich,
  title={{{Rich Feature Hierarchies for Accurate Object Detection and Semantic Segmentation}}},
  author={Girshick, Ross and Donahue, Jeff and Darrell, Trevor and Malik, Jagannath},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={580--587},
  year={2014},
}

@inproceedings{farfade2015multi,
  title={{{Multi-view Face Detection Using Deep Convolutional Neural Networks}}},
  author={Farfade, Sachin Sudhakar and Saberian, Mohammad J and Li, Li-Jia},
  booktitle={Proceedings of the 5th ACM on International Conference on Multimedia Retrieval},
  address={Shanghai, China},
  pages={643--650},
  year={2015},
  organization={ACM, NY, USA}
}

@article{shi2019fast,
  title={{{A Fast and Power-Efficient Hardware Architecture for Non-Maximum Suppression}}},
  author={Shi, Man and Ouyang, Peng and Yin, Shouyi and Liu, Leibo and Wei, Shaojun},
  journal={IEEE Transactions on Circuits and Systems II: Express Briefs},
  volume={66},
  number={11},
  pages={1870--1874},
  year={2019},
  publisher={IEEE}
}

@incollection{li2009mean,
  title={{{Mean Shift Parallel Tracking on GPU}}},
  author={Li, Peihua and Xiao, Lijuan},
  booktitle={Pattern Recognition and Image Analysis},
  pages={120--127},
  year={2009},
  publisher={Springer, Berlin}
}

@inproceedings{shalom2008efficient,
  title={{{Efficient K-means Clustering Using Accelerated Graphics Processors}}},
  author={Shalom, S.A. Arul and Dash, Manoranjan and Tue, Minh},
  booktitle={Data Warehousing and Knowledge Discovery},
  pages={166--175},
  address={Turin, Italy},
  year={2008},
  publisher={Springer, Berlin}
}

@inproceedings{rothe2014nms,
  title={{{Non-maximum Suppression for Object Detection by Passing Messages Between Windows}}},
  author={Rothe, Rasmus and Guillaumin, Matthieu and Van Gool, Luc},
  booktitle={Asian Conference on Computer Vision},
  address={Singapore},
  pages={290--306},
  year={2014},
  organization={Springer, Berlin}
}

@book{litman2017autonomous,
  title={{{Autonomous Vehicle Implementation Predictions}}},
  author={Litman, Todd},
  year={2017},
  address={Victoria, BC, Canada},
  publisher={Victoria Transport Policy Institute}
}

@inproceedings{hosang2017learning,
  title={{{Learning Non-Maximum Suppression}}},
  author={Hosang, Jan Hendrik and Benenson, Rodrigo and Schiele, Bernt},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  address={Honolulu, HI, USA},
  pages={6469--6477},
  publisher={IEEE Computer Society, Washington D.C., USA},
  year={2017}
}

@article{everingham2010pascal,
  title={{{The Pascal Visual Object Classes (VOC) Challenge}}},
  author={Everingham, Mark and Van Gool, Luc and Williams, Christopher KI and Winn, John and Zisserman, Andrew},
  journal={{International Journal of Computer Vision}},
  volume={88},
  number={2},
  pages={303--338},
  year={2010},
  publisher={Springer}
}

@inproceedings{shao2018crowdhuman,
  title={{{CrowdHuman: A Benchmark for Detecting Human in a Crowd}}},
  author={Shao, Shuai and Zhao, Zijian and Li, Boxun and Xiao, Tete and Yu, Gang and Zhang, Xiangyu and Sun, Jian},
  booktitle={Preprint},
  pages={arXiv:1805.00123},
  year={2018}
}

@inproceedings{ellis2010pets2010,
  title={{{PETS2010 and PETS2009 Evaluation of Results Using Individual Ground Truthed Single Views}}},
  author={Ellis, Anna and Ferryman, James},
  booktitle={IEEE International Conference on Advanced Video and Signal Based Surveillance},
  address={Boston, MA, USA},
  pages={135--142},
  year={2010},
  organization={IEEE, Piscataway, NJ, USA}
}

@manual{nvidial4t,
  title={{{Linux for Tegra (L4T)}}},
  author={{NVIDIA Corp.}},
  note={\url{https://developer.nvidia.com/embedded/linux-tegra}},
  year={2019}
}

@incollection{schapire2003boosting,
  title={{{The Boosting Approach to Machine Learning: An Overview}}},
  author={Schapire, Robert E},
  booktitle={{Nonlinear Estimation and Classification}},
  pages={149--171},
  year={2003},
  publisher={Springer, Berlin}
}

@article{cortes1995support,
  title={{{Support Vector Machine}}},
  author={Cortes, Corinna and Vapnik, Vladimir},
  journal={{Machine Learning}},
  volume={20},
  number={3},
  pages={273--297},
  year={1995}
}

@inproceedings{huval2015empirical,
  title={{{An Empirical Evaluation of Deep Learning on Highway Driving}}},
  author={{Huval, Brody et al.}},
  booktitle={Preprint},
  pages={arXiv:1504.01716},
  year={2015}
}

@techreport{karp1988survey,
  title={{{A Survey of Parallel Algorithms for Shared-Memory Machines}}},
  author={Karp, Richard M.},
  institution={University of California at Berkeley},
  address={Berkeley, CA, USA},
  year={1988}
}

@inproceedings{fortune1978parallelism,
  title={{{Parallelism in Random Access Machines}}},
  author={Fortune, Steven and Wyllie, James},
  booktitle={Proceedings of the 10th annual ACM Symposium on Theory of Computing},
  pages={114--118},
  address={San Diego, California, USA},
  year={1978},
  organization={ACM, NY, USA}
}

@inproceedings{qiu2019graph,
  title={{{Graph Convolution and Self Attention Based Non-maximum Suppression}}},
  author={Qiu, Zhe and Gu, Xiaodong},
  booktitle={{International Symposium on Neural Networks}},
  address={Moscow, Russia},
  pages={77--86},
  year={2019},
  organization={Springer, Berlin}
}

@article{song2019improved,
  title={{{Improved Non-maximum Suppression for Object Detection using Harmony Search Algorithm}}},
  author={Song, Yanan and Pan, Quan-Ke and Gao, Liang and Zhang, Biao},
  journal={{Applied Soft Computing}},
  volume={81},
  pages={105478},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{bodla2017soft,
  title={{{Soft-NMS--Improving Object Detection With One Line of Code}}},
  author={Bodla, Navaneeth and Singh, Bharat and Chellappa, Rama and Davis, Larry S},
  booktitle={{Proceedings of the IEEE International Conference on Computer Vision}},
  pages={5561--5569},
  address={Venice, Italy},
  publisher={IEEE Computer Society, Washington D.C., USA},
  year={2017}
}

@inproceedings{liu2019adaptive,
  title={{{Adaptive NMS: Refining Pedestrian Detection in a Crowd}}},
  author={Liu, Songtao and Huang, Di and Wang, Yunhong},
  booktitle={{Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition}},
  address={Long Beach, CA, USA},
  publisher={IEEE, Piscataway, NJ, USA},
  pages={6459--6468},
  year={2019}
}

@inproceedings{salscheider2020featurenms,
  title={{{FeatureNMS: Non-Maximum Suppression by Learning Feature Embeddings}}},
  author={Salscheider, Niels Ole},
  booktitle={Preprint},
  pages={arXiv:2002.07662},
  year={2020}
}

@inproceedings{zhang2017faceboxes,
  title={{{Faceboxes: A CPU Real-Time Face Detector with High Accuracy}}},
  author={Zhang, Shifeng and Zhu, Xiangyu and Lei, Zhen and Shi, Hailin and Wang, Xiaobo and Li, Stan Z},
  booktitle={Proceedings of the IEEE International Joint Conference on Biometrics},
  address={Denver, CO, USA},
  pages={1--9},
  year={2017},
  organization={IEEE, Piscataway, NJ, USA}
}


